Dimension-Accuracy Tradeoffs in Contrastive Embeddings for Triplets, Terminals & Top-k Nearest Neighbors

Metric embeddings traditionally study how to map $n$ items to a target metric space such that distance lengths are not heavily distorted; but what if we only care to preserve the relative order of the distances (and not their length)? In this paper, we are motivated by the following basic question: given triplet comparisons of the form ``item $i$ is closer to item $j$ than to item $k$,'' can we find low-dimensional Euclidean representations for the $n$ items that respect those distance comparisons? Such order-preserving embeddings naturally arise in important applications and have been studied since the 1950s, under the name of ordinal or non-metric embeddings. Our main results are: 1. Nearly-Tight Bounds on Triplet Dimension: We introduce the natural concept of triplet dimension of a dataset, and surprisingly, we show that in order for an ordinal embedding to be triplet-preserving, its dimension needs to grow as $\frac n2$ in the worst case. This is optimal (up to constant) as $n-1$ dimensions always suffice. 2. Tradeoffs for Dimension vs (Ordinal) Relaxation: We then relax the requirement that every triplet should be exactly preserved and present almost tight lower bounds for the maximum ratio between distances whose relative order was inverted by the embedding; this ratio is known as (ordinal) relaxation in the literature and serves as a counterpart to (metric) distortion. 3. New Bounds on Terminal and Top-$k$-NNs Embeddings: Going beyond triplets, we then study two well-motivated scenarios where we care about preserving specific sets of distances (not necessarily triplets). The first scenario is Terminal Ordinal Embeddings and the second scenario is top-$k$-NNs Ordinal Embeddings. To the best of our knowledge, these are some of the first tradeoffs on triplet-preserving ordinal embeddings and the first study of Terminal and Top-$k$-NNs Ordinal Embeddings.

==> header/debug.tex <==
\usepackage{lipsum}

\newcommand{\knote}[1]{{\color{red}$\ll$Kostya: #1$\gg$}}
\newcommand{\vnote}[1]{{\color{red}$\ll$Vaggos: #1$\gg$}}

==> header/todos.tex <==
\iffalse
\subsection{ToDos}
\begin{enumerate}
\item Proofread and polish.
\item Compress the intro to 4-5 pages.
\item Gap Instance for ordinary CSPs (mostly done)
\item {\color{red} Definitions of phylogenetic CSPs, patterns, randomized assignments.}
\item {\color{red} Patterns definitions via $[a,b<c]$.}
\item {\color{red} SDP solution for the general UG reduction.}
\item {\color{red} Remark on non-binary trees.}
\item {\color{red} More than one payoff function.}
\end{enumerate}
\fi
